Understanding the Digital News Consumption Experience During the COVID Pandemic

During the COVID-19 pandemic, people sought information through digital news platforms. To investigate how to design these platforms to support users' needs in a crisis, we conducted a two-week diary study with 22 participants across the United States. Participants' news-consumption experience followed two stages: in the \textbf{seeking} stage, participants increased their general consumption, motivated by three common informational needs -- specifically, to find, understand and verify relevant news pieces. Participants then moved to the \textbf{sustaining} stage, and coping with the news emotionally became as important as their informational needs. We elicited design ideas from participants and used these to distill six themes for creating digital news platforms that provide better informational and emotional support during a crisis. Thus, we contribute, first, a model of users' needs over time with respect to engaging with crisis news, and second, example design concepts for supporting users' needs in each of these stages.

==> graveyard.tex <==
% The research on digital news consumption behaviors is an on-going effort. Bentley et al. \cite{Understanding Online News Behaviors} collected and analyzed the browser logs to find out where did people get news from, what types of news they read and the termporal patterns of news reading. Lee et al. \cite{News sharing in social media: The effect of gratifications and prior experience} applied the uses and gratifications theory to the explanation of news sharing behaviors. Ksiazek et al. \cite{News-seekers and Avoiders: Exploring Patterns of Total News Consumption Across Media and the Relationship to Civic Participation} categorized people into two categories based on their news consumption behaviors: the news-seekers and the avoiders. However, the news consumption under crisis is another story, especially under the current ongoing COVID pandemic.


%voraciously engage with emerging news~\cite{Casero-Ripolles_2020}, and consistent with this phenomenon, visits to news websites increased 28\% in 2020 relative to pre-pandemic averages~\cite{fischer_news_2020}. Thus, as moments of crisis shift people's

%making the consumption experience more convenient and enriched than ever before. On the other hand, people tend to pay more attention to negative news \cite{Effects of Lead Framing on Selective Exposure to Internet News Reports}, and the prevalence of digital news has enlarged the exposure of negative news, which can influence the emotion states of the users \cite{Is the news making us unhappy? The influence of daily news exposure on emotional states; Television news and audience understanding of war, conflict and disaster} and even lead to depression \cite{Associations between COVID-19 related media consumption and symptoms of anxiety, depression and COVID-19 related fear in the general population in Germany}.



% The research on digital news consumption behaviors is an on-going effort. Bentley et al. \cite{Understanding Online News Behaviors} collected and analyzed the browser logs to find out where did people get news from, what types of news they read and the termporal patterns of news reading. Lee et al. \cite{News sharing in social media: The effect of gratifications and prior experience} applied the uses and gratifications theory to the explanation of news sharing behaviors. Ksiazek et al. \cite{News-seekers and Avoiders: Exploring Patterns of Total News Consumption Across Media and the Relationship to Civic Participation} categorized people into two categories based on their news consumption behaviors: the news-seekers and the avoiders. However, the news consumption under crisis is another story, especially under the current ongoing COVID pandemic.

%However, the news consumption experience could change significantly under the crisis time, yet we have little understanding on it. Our research questions are, therefore, listed as follows:


Guided by the data generated by the participants, the research team generated a set of design options, and sketched a news client's interfaces that incorporated the derived designs. We gathered the participants' feedback on the interfaces in the final interview. Based on the results from the study, we propose several design themes towards building a positive news consumption experience during the crisis time.

%Our analysis revealed two significant user needs in the context of news consumption during the crisis: the informational needs and emotional needs. While traditionally news is a piece of information that intended to inform people , we found that people were also seeking emotional support and a sense of connection via reading news during the pandemic. This has presented new challenges to the news platforms : beyond producing information that effectively communicates to the users, news producers should also be considering the potential emotional effect on the users. On the informational side, we need to design interface and mechanisms that helps the user to find relevant news effectively, digest the content and validate the information without too much effort. On the emotional side, we need to be aware of the ``information overload'' while pushing the news feeds, providing resources and solutions towards a positive reading experience, and incorporating social factors.

%how a diverse group of Americans consumed news during one segment of the COVID crisis. Through the interviews and two-week diary study, we identified behavioral changes in their approach to engaging with the news, how people felt about these changes, and their informational and emotional needs in the time of crisis. We also generated design options from the data and evaluated them with the participants. Based on these user needs, design concepts, and feedback on these concepts, we discuss how designers can create news platforms that are supportive of users during times of crisis.

%\subsection{Designing News Platforms for Times of Crisis: Prioritizing Information Needs and Emotional Needs in Parallel}
% The emotional -> equal as informational needs
%two needs show up equally, there's a problem

% Towards building effective resource providing in general
Some of the designs also apply to the general news consumption experience to help people digest and validate the information. For example, we found that several participants would cycle through different sources on a same news topic to understand different perspectives. Aggregating news from different sources can reduce the effort of validating and also provide more comprehensive interpretations of the event. Providing summaries and statistical visualizations also ease understanding and reduce the cognitive load of the readers \cite{hohman2020communicating}. 

%Participants' action-oriented approach to engaging with the news also shifts the definition of what makes content most newsworthy. Under ordinary circumstances, extreme or unusual events might be most notable~\cite{}. However, the user scenario of drawing on locally situated news to make personal decisions suggests that instead of understanding average events, information that can help the user make accurate predictions about their own future will be of more value. This was corroborated by users' interest in seeing news that was relevant to families/friends and news from the local community.



% \begin{table}[h]
% \caption{Problems in digital news consumption during COVID-19}
% \begin{tabular}{|l|l|}
% \toprule
% \multicolumn{2}{|l|}{\textbf{Informational Needs}}                                                                                                                                             \\ \hline
% 1. Finding       & \textit{Lack of easy mechanisms to find the news that matters   }                                                                                                           \\[1.1ex] \hline
% 2. Understanding & \textit{Difficult to extract useful information from a piece of news }                                                                                                      \\[1.1ex] \hline
% 3. Verifying     & \textit{News can be biased and there is no efficient way to check the credibility}                                                                                      \\[1.1ex] \hline
% \multicolumn{2}{|l|}{\textbf{Emotional Needs}}                                                                                                                                                 \\ \hline
% 1. Containing    & \begin{tabular}[c]{@{}l@{}}\textit{The sense of "being a slave to the news" and could not find} \\ \textit{a balance between "getting informed" and "having too much"}.\end{tabular} \\[2ex] \hline
% 2. Coping        & \begin{tabular}[c]{@{}l@{}}\textit{The news were manufacturing outrage and negative effects,} \\ \textit{which could be difficult to cope with}\end{tabular}                         \\[2ex] \hline
% 3. Connecting    & \begin{tabular}[c]{@{}l@{}}\textit{The feeling of isolated and the need to feel connected with} \\ \textit{families and friends}\end{tabular}                         \\[1.2ex] \bottomrule
% \end{tabular}
% \label{tab:problem}
% \end{table}


\subsection{Negative Experiences with Online News}
Despite the public's eager engagement with digital news, the interactive platforms on which it is hosted have introduced new challenges and negative dimensions to people's news-consumption experiences. First, the democratization and diversification of news sources has decentralized editorial control, leading to vast discrepancies in journalistic integrity across news sources.
As a result, not all online news is equally trustworthy, and a large body of prior work has investigated the prevalence of misinformation online (e.g., \cite{Huang2015Connected}), users' perceptions of the credibility of a news source (e.g., \cite{Geeng2020Fake, Flintham2018falling, Hsueh2015leave, wobbrock2019isolating}), and fake news detection \cite{Wu2018tracing, Shu2017fake}. For example, Geeng et al.\cite{Geeng2020Fake} interviewed 25 participants about their experiences interacting with fake news on social media and found that people used various strategies to validate the credibility of article, including investigating its claims, sources, and comments. Taneja and Yaeger \cite{Taneja2019do} analyzed the relationship between an article's trustworthiness and users' engagement, finding that the heavy engagement did not correlate with the high trustworthiness.

%Of particular relevance to the current study, other prior work has examined people's trust in online news specifically in times of crisis. Steelman et al. \cite{Toddi2015what} conducted phone surveys on news trust during five wildfire disasters, finding that family and friends were a more trusted information source than mass media. And an analysis of Pew research surveys \cite{Casero-Ripolles_2020} found that during the COVID-19 outbreak, people's trust in news media and their ability to detect fake news increased. 
%In this study, we also collected participants' strategies to cope with fake news, and came up with design suggestions accordingly.

Second, digital news has introduced new threats to users' mental wellbeing. For example, \textit{negativity bias} \cite{vaish_grossmann_woodward_2008} describes people's tendency to focus more on negative news than positive news. This bias, coupled with algorithms that prioritize content that attracts users' attention, has led to systems that are more likely to surface highly emotional content and make sensationalized content viral~\cite{essay78500}. Other work~\cite{de2020is} and online discussions \cite{reddit_r/coronavirusus_nodate} have similarly concluded that exposure to negative news leads to unhappiness, independently of personality traits. 
%In this work, we are especially interested in how the news consumption affects the mental health as there is a significant amount of negative information about COVID-19. 

%do we need to mention about different types of news consumers (heavy users, incidental encounters, etc)? maybe not too related to the paper findings

Similarly, the digital news ecosystem has produced an explosion of information far exceeding the volume of traditional formats, a phenomenon that has had negative consequences for users' wellbeing.
%During the time of crisis, a person reads news to gather resources and make decisions. However, the issue of today's digital news is that there is too much information, exceeding one's ability to process, adding the stress level. 
In many instances, this excess of news can lead to \textit{information overload}, wherein a taxing amount of information erodes wellbeing and inhibits decision-making \cite{buckland_information_2017}. A 2020 survey found that two-thirds of Americans feel ``worn out'' by the overwhelming amount of news to which they are exposed \cite{gottfried_americans_2020}, and this sense of being overwhelmed routinely leads to anxiety, stress, and the feeling of losing control \cite{EDMUNDS200017}. Further, when overloaded with news, people feel less confident about whether they have found the news they want \cite{PENTINA2014211}, tend to shut down cognitively, will deny the need to continue to consume news \cite{Linda2006the}, and will eventually cut back on news engagement \cite{PENTINA2014211}. The extensive adoption and use of social media has also contributed to the news information overload. Prior studies report several cognitive and behavioral consequences of consuming too much information on social media, including social media fatigue \cite{bright2016too}, news analysis paralysis \cite{Song2017perceive}, and news avoidance \cite{chang2019does}. Given the negative ways in which digital news platforms can impact users' wellbeing, we sought to understand not only how people used these platforms in a crisis, but also how the experience made them feel.

%In this study, we also observed that a large portion of the participants experienced the feeling of ``information overload'', and decreased their consumption time accordingly. From their reflections, we aimed to find design options that could lessen the burden of the consumption experience regarding to too much information.
\subsection{Social Media Use in Crisis}
Social media has introduced new interactive dimensions to reading the news; users can now share and comment on events and even create news themselves. The practice is also referred as ``citizen journalism'' \cite{atton2009alternative}, where public citizens ``\textit{[play] an active role in the process of collecting, reporting, analyzing, and disseminating news and information}'' \cite{bowman2003we}. During crisis events, social media is often an important information source, and it has been studied extensively in this context. Olteanu et al. \cite{Olteanu2015what} identified six ways in which people leverage Twitter during a crisis, including providing emotional support, identifying affected individuals, sharing information about donations and opportunities to volunteer, providing caution and advice, informing others about infrastructure and utilities, and reporting useful information. Qu et al. \cite{Qu2011microblogging} examined the use of Weibo in the aftermath of the 2010 Yushu earthquake in China, showing that people used Weibo platform in ways similar to the Twitter study results. 

Because of the immediacy of social media, people tend to rely on information from these platform to support their risk assessment and decision making. Gui et al. \cite{Gui2017managing} investigated how people used social media to make travel-related decisions during the Zika-virus outbreak. They found that local residents and previous travelers offered crucial resources that were absent from the news and other formal channels. Over the past decade, official organizations have increasingly adopted social media platforms for making announcements during a crisis. For example, the police and fire departments in the cities of US east coast used social media to communicate with residents during Hurricane Sandy, a devastating storm that affected the east coast of the United States in 2012 \cite{Hughes2014online}, as did the University of Canterbury during a massive earthquake in the South Island of New Zealand in 2010 \cite{DABNER201269}. 

As Armstrong and Franklin explain \cite{armstrong2008review}, social media can support collaborative sense-making and the co-creation of knowledge, particularly during time of crisis \cite{Stieglitz2017SensemakingAC, Palen2010avision, Macias2009blog, liu2008search}. Herverin and Zach \cite{Heverin2012use} provide empirical evidence of this phenomenon through their examination of microblogs during three violent crises, and categorized the sense-making practice into six sense-making themes, including \textit{information sharing and seeking, talking cure and understanding the "why"}. 
%Inspired by these previous studies, we sought to understand participants' sense-making experience during their consumption of online information, and identified several needs during the procedure.
Similarly, other work has shown that people use Snapchat to share and consume a wide variety of first-hand accounts of news on the ground, a departure from the perspective offered by traditional media~\cite{Bipat2019ItIN}. Given the central role social media has come to play in the way people experience the news, particularly in times of crisis, we investigated participants needs and design ideas across all of the news and social platforms they engage with. 

\subsection{Situating the COVID-19 Pandemic in the Crisis Literature}
Every crisis is different, and the way in which people experienced the COVID-19 pandemic may or may not align with people's experiences of other crises. According to the sociology of disaster research (p. 50 in \cite{Perry2005WhatIA}), crisis events can be categorized along several dimensions \cite{Olteanu2015what}, including the type of hazard (e.g., natural vs. human-induced), temporal development (instantaneous vs. progressive), and geographic spread (focalized vs. diffused). Previous research has found that information flow varies substantially across these different crisis types \cite{Olteanu2015what, Kanhabua2013understanding}. In this paper we specifically exmaine the COVID-19 pandemic, a long-lasting crisis with global spread. In addition to its accompanying public health and economic impacts, the pandemic was characterized by ``stay-at-home'' orders in many areas that restricted physical interactions. 

In the 15 months since COVID-19 was first identified, the scientific literature has rapidly sought to document the crisis and people's experiences with it, including investigations of news consumption. Research conducted by Bruce et al. \cite{NBERw28110} analyzed over 20,000 COVID-19 related news articles, finding that 91\% of major U.S. media outlets were negative in tone versus 54\% for non-U.S. major sources and 65\% for scientific publications. The disproportionately large portion of negative news together with the increase of the news consumption during the COVID-19 pandemic \cite{Casero-Ripolles_2020}, has led to information overload \cite{info11080375, Austin2012HowAS} and been implicated in increases in mental health struggles, including depression and anxiety \cite{GarfinThe2020, Bendau2020, Gaomental, chao2020media, Riehm2020associations, excessive}. 

Yet, prior work has also shown that people's engagement with COVID-related news has had many benefits. Liu \cite{liu2020COVID} found that consuming COVID-related news led people to take preventative measures and enabled them to protect themselves from contracting the virus. Other work has helped to make sense of people's patterns of engagement with COVID-related news. For example, prior work has shown that people who trust left-leaning American news sources, such as CNN, tended to engage in less risky activities than people who trust right-leaning American sources, such as Fox News \cite{Zhaoe003323}. Other literature has found that people became more likely to seek out local news when the COVID pandemic began \cite{castriota2020national}, and that people become more likely to look for actionable news items during crises generally \cite{howpetrun, Olteanu2015what} (two findings that also emerged in the current study).

To date, this prior literature has primarily included surveys and interviews to understand people's experiences consuming COVID-19 news and information. We expand on this foundation, first, by capturing \textit{in situ} data about news consumption using diary methods. We then draw upon this foundation to investigate how to design a positive experience for digital news consumption under such a crisis.
